How Are Learned Perception-Based Controllers Impacted by the Limits of Robust Control?

The difficulty of optimal control problems has classically been characterized in terms of system properties such as minimum eigenvalues of controllability/observability gramians. We revisit these characterizations in the context of the increasing popularity of data-driven techniques like reinforcement learning (RL), and in control settings where input observations are high-dimensional images and transition dynamics are unknown. Specifically, we ask: to what extent are quantifiable control and perceptual difficulty metrics of a task predictive of the performance and sample complexity of data-driven controllers? We modulate two different types of partial observability in a cartpole "stick-balancing" problem -- (i) the height of one visible fixation point on the cartpole, which can be used to tune fundamental limits of performance achievable by any controller, and by (ii) the level of perception noise in the fixation point position inferred from depth or RGB images of the cartpole. In these settings, we empirically study two popular families of controllers: RL and system identification-based $H_\infty$ control, using visually estimated system state. Our results show that the fundamental limits of robust control have corresponding implications for the sample-efficiency and performance of learned perception-based controllers. Visit our project website https://jxu.ai/rl-vs-control-web for more information.

==> sections/controls-background-rough.tex <==
\section{Controls background rough}
\note{probably want to move some of this to intro}
% Much of the research in the learning for control community has focused on characterizing \emph{achievable upper bounds} on the performance of learning based control strategies.  While such upper bounds are common in the literature, \emph{lower bounds} are few and far between. For model-free RL methods as applied to the Linear Quadratic Regulator, such lower-bounds can be found in \citep{tu2018gap}, where the authors derive asymptotic lower bounds on the number of samples needed by both the least-squares-temporal-differencing estimator for policy evaluation, and policy gradient methods for policy improvement.  In \citep{simchowitz2018learning, simchowitz2020naive} information-theoretic lower bounds \citep{tsybakov2008introduction,duchi2016lecture} are derived for arbitrary estimators, which in turn are used to show the optimality of certainty equivalent control for the LQ problem.  We note that in both cases, such lower bounds are only available for \emph{full-state} observation settings.  Although lower bounds are uncommon in the learning based control literature, a rich set of results on the fundamental limits of control can be found in the robust control literature.  For example, if a system has an open-loop unstable pole $p$ and unstable zero $q$, and these are close in value, then this lower bounds the $\mathcal{H}_\infty$ norm of the complementary sensitivity function as $\Omega(\frac{1}{|p-q|})$ \citep{doyle2013feedback,leong2016understanding}. To the best of our knowledge, no investigation of the effects of such fundamental limits on learning-based control methods exist -- this may be due to the fact that many demonstrations of learning-based control methods are on over-engineered systems for which sensing and actuation are not an issue.  However, as learning  systems move from the lab into the real world, systems with full-sensing that are overly-actuated may become prohibitive or impossible to build.  In this research thrust, using perception-based control as a testbed, we initiate a study on the \emph{fundamental limits of robust learning-enabled control}.  Our objective is to understand how the underlying robustness/fragility of a control system imposes fundamental limits on the robustness and  sample-complexity of learning-enabled control.

% \textbf{Significance and Impact:} Understanding how the robustness/fragility of a control system affects the robustness and sample-complexity of learning-enabled control algorithms implemented on it will yield critical design insights, and has the potential to be as transformational and impactful on the field as the Bode Integral and Waterbed formula has been on the field of robust control.

% \textbf{Background:} \note{can probably recycle a lot of this for an intro section to the stick-balancing problem, but need to flesh out the detail a little bit more using \citep{leong2016understanding}.} We propose using the ``stick-balancing'' example from \citep{leong2016understanding,doyle2013feedback}, shown in Fig.~\ref{fig:stick}, to initiate our study.  This system features two important properties: (i) it unstable, with open-loop unstable pole $p\propto 1/\ell^{1/2}$, for $\ell$ the length of the stick and (ii) it is non-minimum phase, with open-loop unstable zero $q\propto 1/(\ell-\ell_0)^{1/2}$ where $\ell_0$ denotes the \emph{fixation point} on the stick where the eye is looking (see Fig.~\ref{fig:stick}).  We can can make the control problem \emph{quantitatively} more difficult by letting $\ell_0\to 0$ (i.e., by letting the open-loop unstable zero $q\propto 1/(\ell-\ell_0)^{1/2}$ approach the open-loop unstable pole $p\propto 1/\ell^{1/2}$) (follows from applying max-modulus theorem to the complementary sensitivity function, see \citep{leong2016understanding,doyle2013feedback}) to show that 
% \begin{equation}\label{eq:fragility}
%     \log \norm{T(s)}_{\infty} \geq \log\left|\frac{p+q}{p-q}\right|,
% \end{equation}
% where here $\norm{T(s)}_\infty$ denotes the $H_\infty$ norm of the complementary sensitivity function $T(s)$ mapping sensor noise $n$ to controlled output $z$.  We emphasize that the bound \eqref{eq:fragility} holds \emph{for all possible controllers}, including the optimal $H_\infty$ controller, and thus represents a fundamental lower bound on achievable performance.

% \begin{wrapfigure}{r}{.26\textwidth}
% \includegraphics[width=.255\textwidth]{l4dc/figures/stick-setup.pdf}
% \caption{Custom ``stick-balancing'' PyBullet environment \citep{coumans2016pybullet}.  The controller view is head on (left inset); to replicate shortened fixation point, we make a top portion of the rod invisible (in black).}
% \label{fig:pybullet}
% \end{wrapfigure}

% We will use this system, and crucially, its ability to quantitatively tune the fragility \eqref{eq:fragility} of the underlying control problem by adjusting the fixation point $\ell_0$, to study fundamental limits of learning-enabled control.

% \paragraph{Research Challenge I: Empirical Characterization of Fundamental Limits} It is important that the problems we study capture meaningful empirical phenomena.  To that end, this research challenge will seek to identify, through careful use of simulation and hardware experiments, empirical tradeoffs and fundamental limits of learning-enabled control, as they are related to the underlying properties of a control system.






% \paragraph{Technical Approach I: A control/perception robustness tradeoff}



% As a starting point, we consider studying the robustness and sample-complexity of (perception-based) RL algorithms on the inverted pendulum problem described above.  To do so, we developed a custom ``stick-balancing'' environment in PyBullet \citep{coumans2016pybullet}, illustrated in Fig.~\ref{fig:pybullet}.  An inverted pendulum is actuated by moving along a sliding track (in cyan): the perception-based controller is given a \emph{head on} view, as shown in the inset.  To mimic varying fixation points, we make portions of the rod invisible to the controller, displayed in black in the simulation environment. 


% This simple experiment suggests that for this system and algorithm, sensing location has a significant impact on sample-complexity.  We will use the inverted-pendulum testbed, with its quantifiable degree of control difficulty as captured by the fixation length $\ell_0$, to explore other tradeoffs in the learning-enabled control space.  For example, we will explore if systems that are fragile to measurement noise, as captured by the bound \eqref{eq:fragility}, are inherently sensitive to distribution shift.  We discuss why we believe such a tradeoff may exist at the end of the next Technical Approach. Once such compelling tradeoffs have been identified in our simple setup, we will work with our collaborators in the GRASP lab to examine whether they carry over to more realistic real-world robotic tasks, such as robotic manipulation and navigation.  We are also interested in determining the theoretical underpinnings of such phenomena, as we formalize next.


